Community Networks and Sustainability: a Survey of Perceptions, Practices, and Proposed Solutions

Community network (CN) initiatives have been around for roughly two decades, evangelizing a distinctly different paradigm for building, maintaining, and sharing network infrastructure but also defending the basic human right to Internet access. Over this time they have evolved into a mosaic of systems that vary widely with respect to their network technologies, their offered services, their organizational structure, and the way they position themselves in the overall telecommunications' ecosystem. Common to all these highly differentiated initiatives is the sustainability challenge. We approach sustainability as a broad term with an economical, political, and cultural context. We first review the different perceptions of the term. These vary both across and within the different types of stakeholders involved in CNs and are reflected in their motivation to join such initiatives. Then, we study the diverse ways that CN operators pursue the sustainability goal. Depending on the actual context of the term, these range all the way from mechanisms to fund their activities and synergistic approaches with commercial service providers, to organizational structures and social activities that serve as incentives to maximize the engagement of their members. Finally, we iterate and discuss theoretical concepts of incentive mechanisms that have been proposed in the literature for these networks as well as implemented tools and processes designed to set the ground for CN participation. While, theoretical mechanisms leverage game theory, reputation frameworks, and social mechanisms, implemented mechanisms focus on organizational matters, education and services, all aiming to motivate the active and sustained participation of users and other actors in the CN.

==> sections/CN_sustainability.tex <==
\section{Community networks and the sustainability question}\label{network_sustainability}

The survival of CNs as complex and multi-leveled structures depends on a number of reasons. To identify those reasons it is important to look at the interaction of individual actors, their level of participation and the exact models and mechanisms followed. While some combinations of efforts lead the CN to great success and expansion of the network others may lead to failure and depletion. There are clearly no recipes on how to reach one end or the other. Hence, it is interesting to identify the different perceptions in moving towards a sustainable CN.
 
These perceptions have risen from the conceptual framework of sustainability developed by Fuchs in netCommons deliverable \cite{NETCOMMONS_D2_1} and the case studies and interviews from CN participants in \cite{NETCOMMONS_D2_2} that build and complement th work in \cite{NETCOMMONS_D2_1}.
 
% \textit{These perceptions have risen from the conceptual framework of sustainability developed by Fuchs (D2.1) and the case studies and interviews from CN participants in [D2.2] that build and complement th work in (D2.1). These were both held within the framework of netCommons project.  The case studies and interviews involve a wide variety of CNs located in the EU, notably in the UK and Greece: Consume.net in East London; Free2Air in East London; Digcoop in East London; B4RN in Lancaster; Kinmuck in Aberdeenshire; I4free network in Trizonia, near Nafpaktos, Greece; and the Sarantaporo network in northern Greece.}
 
 
\subsection{Sustainability of a CN}
Sustainability is a multifaceted concept used to study a variety of systems \ie biological, socio-cultural, technical. Its actual definition is established in accordance with the system of interest. In general, the great sustainability challenge revolves around identifying and understanding the way that a system can function in the present and endure in the future \ie develop in a sustainable way. Sustainability is not a specific goal per se but a continuous process to reach a goal. Its first acknowledged aspect refers to environmental sustainability and it was defined as the process of a sustainable development that should be able to satisfy current human needs without compromising the fulfillment of needs for the future generations (United Nations World Commission on Environment and Development (WCED) 1987). In recent years, the definition has developed to include three pillars of sustainability environmental, social and economical (World Summit on Social Development, 2005).  
In the context of a CN, sustainability is seen as a multi-dimensional concept of \textit{economic, political and socio-cultural} aspects \cite{NETCOMMONS_D2_1} like any other community of people. 
 
 
 \subsection{Perceptions and common themes}
 
 
  Following the empirical research in \cite{NETCOMMONS_D2_2}, the perceived dimensions show that a) \textit{economic sustainability} concerns funding and resourcing, the size of the community, and time b) the understanding for \textit{political sustainability} is relevant to organizational and legal issues, as well as open structures, and c) \textit{cultural sustainability} contemplates the sense of belonging, community identity and spirit and communitarian practices. 
 

The different dimensions of sustainability are analyzed in detail below.\\ % risen from the case studies in [D2.2].  
 
\subsubsection{Economic sustainability} 
 It is primarily based on the personal efforts of the CN's participants. The results of the comparative research showed that in a number of cases (Consume, Free2Air, i4free) personal efforts by a small number of people or even a single individual were instrumental for the deployment and take off of the network. However, there is a range of models that diverse actors understand as sustainable.
 
\begin{itemize}
\item \textbf{Requirements:}
Certain conditions have been identified as crucial for the development of a sustainable network. Firstly, the size of the community of the network plays a significant role in the economic sustainability of the initiative, in the sense of providing a critical mass of users/members who can either provide subscriptions or contribute their resources. Secondly, time is another valuable resource. Such CN
initiatives depend by definition on volunteers who are prepared to give up their time and contribute
to various aspects and stages of the process. Thirdly, the access to funding is crucial for the network's economic sustainability.

\item \textbf{Non profit vs for profit models:} 
 Considering the \textit{profitable character} of the network, there are two different economic models. On the one hand, the sustainability model has to do with maintaining an alternative character and bypassing commercial interests, particularly those of the big providers (e.g. Consume, Free2Air, B4RN, i4free). This model perceives community networks as grounded on commons, communitarian practices and not-profit initiatives. On the other hand, sustainability is simply a matter of providing a good service, and this can be realised better through commercial arrangements, albeit with small commercial providers, rather than the big telcos (e.g. Kinmuck). This conception is based on for-profit provision but by small- and medium-sized enterprises. The main economic contradiction underlying community networks models appears to be one between community economy and commercial for-profit provision.
 
 The provision of Internet connectivity by community networks is significantly cheaper and often better quality and faster than commercial alternatives, if they exist. Subscriptions then are relatively low and do not jeopardise affordability. It is important to note here that, in sharp contrast to commercial for-profit provision, the non-profit character of community networks contributes to their sustainability in various ways. First, subscriptions are affordable. This creates a virtuous circle: the more affordable access to the community network is, the more users will join; the more users join, the larger the pool that contributes to the financing of the network helping therefore to maintain subscriptions affordable. Second, this non-profit funding model of community networks brings the community closer together and this in turn increases the commitment of the community to the network. Rather than (higher) network subscriptions creating profits which then go into benefiting primarily the shareholders of commercial for-profit providers, the link between financial (and other, for instance time) contributions by community members and the development of the community network is more direct and visible to the community in question.
  The non-profit character of community networks improves their economic sustainability and strengthens community ties and commitment to the initiative.
It is also worth stressing that many communities value inclusiveness more than profitability. Some communities have ways to provide connection even to those who could not afford it (e.g. B4RN). Equally, fairness is another aspect that some pricing policies reflected as is the case of B4RN where there are different pricing schemes for residential users, small enterprises and bigger businesses, the latter two considered as heavier Internet users.
 
 \item \textbf{External vs internal funding models:}
 Economic perceptions in terms of \textit{funding practices} can also be distinguished. As far as funding is concerned, there are two possible ways of income a) receive funding resources from entities external to the network or b) from the network's own resources.
 
 There are examples of communities that tried to access local or national funding (in the case of B4RN, their bid was subsequently withdrawn and put into a larger regional pool). However, it is suggested \cite{NETCOMMONS_D2_2} that financial sustainability requires a subscription model and the funding of the network from community-owned resources. It is not simply the case that some community networks found potential access to local, national or European funds too difficult and demanding, often not tailored to such initiatives, uncertain, and too bureaucratic, but it is the belief that the funding of a community network from own-resources is more reliable and sustainable (e.g. B4RN), as it precludes dependence on external funding which might not materialise or, given that it has a fixed term, it might put at risk the subsequent development and maintenance of the network when it finishes. Internal funding from own resources, if possible, is preferred within the CNs. 
 
 
 External funding sources may be \cite{NETCOMMONS_D2_4}

\begin{enumerate}[label=\alph*)]
\item \textit{Donations from external supporters:} Community Networks are often financed through crowd-funding projects or direct, regular or one-time, donations (\ie Freifunk.net).
%Freifunk.net offers a good example of attracting such support through a dedicated non-profit organization, which is meant to require as little as possible (voluntary) effort. For this reason, it has a relatively small number of regular members and a large circle of supporting members, which can all participate in the annual general meeting. The membership includes a “fee of either 60 EUR (or more) per year to the Association's account as annual sponsor membership, or the monthly equivalent of 5 EUR (or more) for sustaining membership.”1

\item \textit{Funding from institutions:} Receive hardware and equipment from the Free/Open Source
Software Society (GFOSS) and funding by national or European projects (\ie Sarantaporo.gr). 
% A good example of such a community network is Sarantaporo.gr CN. They managed to establish a network that offers today broadband Internet access to 14 villages in a rural area in Greece with limited or no fixed network connectivity. This particular network was built initially by a small team of young activists who received hardware by the OpenWifi call of the Greek Free/Open Source Software Society (GFOSS), and funding by the EU project CONFINE to develop a community network as a “testbed” for experimentation on future Internet technologies (Navarro et al, 2016).

\item \textit{Access to public infrastructure:} Being non-profit, official or unofficial organizations, CNs are often granted access to public infrastructure in favorable terms (\ie Sarantaporo.gr). Public buildings can be used to place and store the network's equipment. However, cases in which CNs are treated unfairly in comparison with traditional
providers are also present (\ie guifi.net). 

%\textit{Being non-profit, official or unofficial organizations, CNs are often granted access to public infrastructure in favorable terms. For example, Freifunk.net nodes are often placed on churches and the Sarantaporo.gr network has been offered free Internet access by the University of Applied Sciences in Thessaly (see D1.2 and D3.1). However, there are also cases in which CNs are treated unfairly in comparison with traditional providers as in the case of Barcelona’s access network. The guifi.net Foundation and its local partner, the eXO association (see D1.2), have discussed the terms of usage of the public city-wide WiFi infrastructure and the city fibre infrastructure. In both cases, the inherited situation is that both services were privatised (a concession to private operators, with strict conditions and long terms) that prevent the open access to this infrastructure in reasonable terms. Therefore, the BCN-WiFi2 infrastructure consisting of about 600 Access Points (a large number in the statistics for such a large city, but clearly unpopular service with usability, speed, coverage and reliability problems) is privately managed. The public fibre infrastructure and the conducts are also under a long-term concession that provides service to the municipality but impedes any other practical usage of that infrastructure. Despite the obstacles in deploying infrastructure and services in the city of Barcelona, guifi.net around Spain benefits from more favorable policies in terms of access to public infrastructure (e.g., for laying out fibre cables) compared to other countries. }



\item \textit{Market-based policies:} 
It is often the case that economic sustainability is linked to for-profit activities and there are
commercial networks that indeed rely on such policies ranging from standard pay per use contracts, like in the case of some of the FFDN networks, advertising other added value services to external customers. When the policies reach out to external customers, this type of funding can be considered external. 


%ranging from standard pay per use contracts,like in the case of some of the FFDN networks, advertising other added value services to external customers. Also, Kinmuck network in Aberdeen, which is served by a technical enterprise, which charges standard contracts in an area where there is no Internet (they provide fibre infrastructure).}

\item \textit{Partnerships with local authorities:} 

A good model for community networks seems to be a hybrid/co-operation of commons/public
service with civil society/municipality, in which civil society projects co-operate with
municipalities \cite{RePEc:ehl:lserod:29461}, \cite{powell2006going},\cite{powell2008wifi}. So, the survival problems
of alternative media may be limited if one can find models in which municipal power and civil
society commons are not seen as opposing each other, but acting cooperatively as antidotes to the mainstream and profit-making media outlets. 

The guifi.net Foundation has developed a cooperative infrastructure sharing model (the “Universal”
deployment model) that develops over the Directive 2014/61/CE on broadband cost reduction of the EU\footnote{\url{https://ec.europa.eu/digital-single-market/en/news/factsheets-directive-201461ce-broadband-cost-reduction}} and the infrastructure sharing concept of ITU\footnote{\url{https://www.itu.int/ITU-D/treg/publications/Trends08_exec_A5-e.pdf}} to regulate the details of
how municipalities and counties can regulate the use of public space by private, government and
civil society in a sustainable manner. The proposal is written as a template municipal ordinance to
be used by municipalities to regulate this complex aspect correctly and fairly and, therefore, reduce
the barriers created by uncertainty in these topics that usually escape the knowledge of municipal
governments.

\end{enumerate}




Moreover, internal resources commonly used in CNs, may refer to
\begin{enumerate}[label=\alph*)]
\item \textit{Voluntary contributions from members:} This is the most common source of contributions based on which many existing Community Networks have managed to thrive, like AWMN in Greece, Ninux.net in Italy, Wlanslovenja, and Freifunk.net in Germany.
The networks reach a significant scale relying mostly on its own members’ investments in
time, effort, and equipment. To achieve this level of participation (\ie Freifunk), these networks usually develop strong feelings of
community and intrinsic motivations related to the commitment toward a more democratic, private,
secure, and neutral Internet offering affordable access to all.

\item \textit{Commons-based policies:}
Some of the sources of financial support (\ie donations, voluntary contributions \etc) are one way or another not guaranteed, and they
make long-term strategic planning difficult. They could also lead to disagreements and conflicts
between members on its distribution inside the network, especially if there are not well-defined
decision-making processes.
When the infrastructure costs are high, it is often the case that CNs are organized around formal
organizations such as NPOs and broadband co-operatives in which large numbers of local community members join and pay membership fees in order to set up the network (Dutch networks, B4RN). 
They can also develop unique models combining voluntary and professional services in a commons-based approach. As we have seen in section II, guifi.net has focused on building and managing network infrastructure in a way that is sustainable, fair and non-profit, based on a novel compensation scheme \cite{Baig:2016:MCN:2940157.2940163}. 

%such as the Dutch broadband co-operatives, studied by Sadowski and others in 2014, in which large numbers of local community members join and pay membership fees in order to set up fibre networks. The network B4RN in the area of Lancaster in the UK (discussed in detail in deliverable D2.2) is another example. Guifi.net has developed a unique model combining voluntary and professional services in a commons-based approach on building and managing network infrastructure in a way that is sustainable, fair and non-profit, based on a novel compensation scheme (Baig et al, 2016). The participants who use a significant amount of resources from the infrastructure commons are obliged to sign an agreement for economic activities and for the participation in the compensation system.



\item \textit{Market-based policies:} In this case the commercial activities are developed for network users only and they do not target external customers.  

\item \textit{Incentive mechanisms:} Another strategy in ensuring the economic sustainability of a Community Network is making it
attractive in the first place. The description of the vision and key principles, the public image, the
availability of Internet connectivity or not, the existence of local services of good quality, the
participation rules, are some of the important aspects that motivate people to join a CN either as contributing members or simply as users. 

\end{enumerate}



\end{itemize} %economic sustainability bullets a) requirements, b) models 

\vspace{3mm}

\subsubsection{Socio-cultural sustainability} It is predominantly understood as a spirit of social cohesion and common identity or, at least, as a spirit of sharing common resources. 




\begin{itemize}


\item \textbf{Requirements:} The socio-cultural sustainability of a CN, requires the satisfaction of certain conditions within the community. 

The presence of a strong relatively closely-knit community is a necessary but not sufficient condition for the take-off and subsequent success of community network initiatives. In turn, through the process of setting up and running the network the community is brought closer together and in this sense community ties are further strengthened, whilst Internet connectivity brings the community closer to other parts of the society. In short, social cohesion is therefore enhanced.

Good community relations also matter. Knowing the people in the community well can help resolve any disagreements, conflicts and soften intransigence (e.g. B4RN). Conversely, mistrust in the community adversely impacts upon the sustainability of the network (e.g. i4free).

The community needs to have identified specific needs that the initiative will address. To start with, a basic need is Internet connectivity and possibly at a later stage specific community-services. Put differently, there has to be demand in the community.

Moreover, the community has to be resourceful. Various resources are essential and they include: a community leader who can bring the community behind the project, and technology leaders who will design the network. Added skills are desirable such as people with a good knowledge of accounts and law. The more people are trained and willing to take on leadership roles the better it is for the network. This can counter problems when some leaders have to move on and cannot commit anymore to the same degree.

Experimentation and knowledge play a central role in many of the CNs examined. Very often the technology leader at least is regular contact with other leaders in other communities with similar initiatives underway. Knowledge exchange and sharing of experiences can contribute to the sustainability of the network. Many actors attach great importance in involving the young generation and provide motivation to them to build skills and transfer them in building other community networks.

While the presence of relevant, mostly technical, knowledge is an important precondition for the initiation of a community network initiative, not all CNs are confined to so-called geek-publics. Although some might have started as communities of geeks (e.g. Consume), all the networks studied for the present deliverable strived to reach out to the general public of non-geeks and non-techies. Still, the passing down of technical knowledge, the sharing of experiences and the support of other similar initiatives, as well as, the acquisition of new technical knowledge and capabilities are all key elements for the sustainability of community networks. 


\item \textbf{Strong vs weak commitment models:}
Depending on whether the aforementioned conditions are satisfied or not, the following socio-cultural sustainability models can be identified.

Communitarian practices and philosophical concerns for the commons in general are often additional features of the communities (e.g. Digcoop, Consume, Free2Air). Commitment, solidarity and trust are key ingredients for a socio-cultural sustainability model and their absence is detrimental to it. However within the CN, one can also find cases of people that do not abide to these characteristics. Network members that prioritize and value individual profit instead of solidarity and community spirit are in many cases present. They take the role of -resource and connectivity- consumers and contribute poorly or not at all. 
The problem identified, namely free-riding in peer initiatives and their reliance on the efforts of the very few for the benefit of the many, is a socio-cultural contradiction at the heart of community networks. 



\end{itemize}



\vspace{3mm}

\subsubsection{Political sustainability} The idea of empowerment, active ownership of resources and data, and control of one’s own communication needs, often linked with the idea of bypassing dominant commercial providers, are the basis of CN structure. They offer an open structure, whose management, operation, experimentation and lack of censorship are hugely important.

\begin{itemize}

\item \textbf{Requirements:} Organisational aspects are a locus of cultural contradictions of community networks, as in some cases they can operate against sustainability. A suitable organisational form, addressing economic aspects but also being democratic and targeted towards serving community interests is thus perceived of as essential for sustainability.

Legal aspects can be seen as ingredients potentially threatening sustainability. The case of Sarantaporo, operating a non-profit community network, possibly faces legal challenges based on the Greek regulatory framework, which does not distinguish between the regulation of for-profit and non-profit network providers.

Moreover, CNs need to be kept synchronized and follow current technological
developments. Technological changes at the level of applications might make
the choices of the community network obsolete. The proliferation of
sophisticated applications on the Internet, and the lower cost of storing such applications on cloud,
as opposed to local servers, create further tensions on community networks. CNs have to be kept up-to-date with current and future technological needs of their members but also, maintain their unique characteristics (\ie local character).

\item \textbf{Privacy-aware vs privacy-unaware models:} 
The contradiction here is one between the potentially more open and privacy-friendlier character of community networks, and the closed environment of commercial for-profit networks where surveillance practices are deeply entrenched features for commercial and political reasons. Awareness around privacy has increased in recent years, in particular following the Snowden revelations, and the open privacy-respecting alternative that community networks promise might well increase their attractiveness and contribute to their growth and expansion. The cases examined have generally provided opportunities for user active involvement in managing their data and have kept central user data storage and control at a minimum. 
 However, the contradiction between data control/privacy and data ownership by big corporations, such as Facebook, remains in the cases where community networks are used only for
free or low-cost Internet access for the purpose of deploying these large corporate platforms.







 \end{itemize}







%\textit{A regulatory framework embracing community networks should be a two-tier framework : (a) recognizing the legal status per se of the common pool resource [community network] as a common good and embedding high level rules as to its governance, and (b) recognize the rights of producers-users to contribute work and resources without imposing regulatory burdens. Access providers to the network should be able to cover expenses for the provision of scarce resources, such as access to the Internet or support.} (George Klissiaris, interview, 29 November 2016).


%Some of these issues echo the situation in the UK:


%\textit{There are still no legal issues with setting up a community network, but increasingly there is an anxiety that doing so will lead to an exposure of risk for those sharing internet gateways, setting up social enterprise and competing for resources and attention of publics. The Digital Economy Act, passed at end of the Labour government, was very disruptive in terms of perceptions of how more exposed we could be to claims of damages from copyright holders and police investigations of cyber crime...60\% of the material exchanged over the internet is still peer-to-peer but it all goes via commercial intermediaries. The spectre of risk has taken the fun out of sharing for most people who prefer to outsource their media servicing tasks rather than face responsibilities of DIY.} (James Stevens, interview, 30 September 2016).


%Perceptions of sustainability of community networks are also influenced by current technological developments. When Digcoop started, for instance, there was limited access to the Internet. Closing the digital divide and promoting digital accessibility were very strong arguments at the time but these have lost their strength, even though the issues are still valid. Internet access has increased, its costs have generally fallen and the entry into the market by various commercial providers threatens the viability of community networks.Technological changes at the level of applications might make the choices of the community network obsolete. Our interviewees have expressed awareness that local applications do not make as much sense as it used to be the case. The proliferation of sophisticated applications on the Internet, and the lower cost of storing such applications on cloud, as opposed to local servers, create further tensions on community networks.







% Sustainability in political, socio-cultural and economic aspects. [ Ch.1.1 from D2.2, possibly material extracted from D2.1  ]


%\begin{itemize}
%\item Definition of sustainability and its multiple aspects [ Ch.1.1 from D2.2, possibly material extracted from D2.1  ]
%\item Perceptions, common themes [Ch.3 from D2.2]
%\item  inputs : D2.1, D2.2 
%\end{itemize}
%As we have seen in the previous section []%[\ref{network_sustainability}], 
%the sustainability of community networks is

 
 
%(and the overall economic model of CN, including capex, opex, contribution, consumption, balances) and then discuss about incentives to participate in the overall model (the cost of deploying and maintaining the infrastructure and connectivity). For me the sustainability model describes the complete model,










==> sections/stakeholders_incentives.tex <==
\section{CN STAKEHOLDERS AND INCENTIVES FOR PARTICIPATION} 


 Originating from the fact that CNs are complex socio-technical systems, built and operated by humans, that combine the technological infrastructure with the multiple social dimensions [C. Fuchs[3], M. Gurstein [4]], it possible to say that they form a kind of society [Schuler[5]] whose physical existence is based on technological elements, i.e., infrastructure, software.  In fact, the technical infrastructure itself can be considered as a result of social interaction among network participants and as an ex-ante condition for further political, socio-cultural and economic interactions among the community members. 

As we have seen in the section \ref{network_sustainability}, the sustainability of community networks is a multi-dimensional (political, socio-cultural, economic) concept which is highly dependent on CN user participation. 

It is important to note that network participants are not homogeneous. Different types of users weigh differently their participation depending on their interests, status, obligations, goals and motivations. This heterogeneity can be expressed using four types of stakeholders \textit{Volunteers, Users, Professionals, Public administrations} as they were primarily established in guifi.net. Each stakeholder possesses its own incentives for participating. 

In general, the incentives for joining a CN, can be distinguished according to the dimensions adopted for the concept of sustainability. They can be \textit{politically, socio-culturally or economically} oriented.
\begin{figure}
\centering
   \includegraphics[width=0.95\columnwidth]{figures/stakeholder_incentives}
    \caption{Primary participation incentives per stakeholder type.}
    \label{incentives_st}
\end{figure}
%\subsection{CN Incentive Dimensions}
%\subsubsection{Political}
%\subsubsection{Socio-cultural}
%\subsubsection{Economic}
%\subsection{Stakeholders}

\subsection{Volunteers}\label{volunteer}%\textit{\color{red}{Definition and incentives.}}
The term \textit{volunteer} is used to define an individual or a group activated to offer their services for a purpose without desiring any compensation in return. In the context of CNs, volunteers are the people that offer their services for the creation of a CN. They are the initiators of the CN project. Their interests reside in aspects of \textit{neutrality, privacy, independence, creativity, innovation, DIY, or protection of consumers' rights}.

Almost always, (a subset of) these people retain their interest in the network after its original deployment phase, holding the responsibility for the operation and maintenance of the CN~\cite{DBLP:journals/corr/abs-1207-1031}. And more often than not, they take an active role in the network expansion, either through helping with the technical matters and/or organizing informational and training events for potential participants.

%The motivating factors that urge volunteers to get involved with a CN span across different dimensions. The interest of creating a network independent from the current telecommunication model resides in supporting the idea of net neutrality i.e. avoiding data discrimination, privacy of user data reside within the network, independence i.e. avoiding the dependency on large telecom networks for their communication, creativity i.e. the need to build something fulfilling one's personal aspirations, innovation i.e. implementing a novel idea and becoming pioneer, Do It Yourselfs (DIY) i.e. being inspired to follow the DIY paradigm or even protecting consumer's rights i.e. by following an alternative model for providing services. 

Volunteers usually form the core team responsible for the management and operation of the network. Managing the network infrastructure refers to designing, planning, developing and maintaining the network. These are implemented by organizing and coordinating the efforts of participants, finding resources or even resolving issues that arise from the use of the network i.e. technical problems, conflicts, etc. In their effort to regulate all these matters, volunteers utilize software tools for the network infrastructure and governance tools for the participation of users. Also, it is not uncommon for
volunteers to create a legal entity to represent the network to third parties (i.e.,
government, third party organizations, companies, Internet Service Providers (ISPs) providers). This lets them have a voice and interface with third parties on legal and regulatory matters, but also get involved in financial transactions (e.g., user subscriptions, fund raising, purchase of equipment).

The volunteer groups usually comprise of people that cumulatively possess knowledge and expertise over a wide set of areas~\cite{aichele2006wireless}:

\begin{itemize}
\item{In technical matters concerning the development of a computer network, ranging from installing and fine tuning antennas to configuring connections, IP addresses and network routes, and troubleshooting problems at both hardware and software level;}
\item{In legal matters such as national and international legislation around technology and civil law, including the provisions of licenses, regulation status, and possible agreement frameworks for the operation of the network;}
\item{In potential sources of funding, primarily from public administrations at national and European Union level.}
\end{itemize}

The volunteer groups typically involve technology enthusiasts, radio amateurs, hackers, activists, and academics. 
Their motives have a strong bias towards political and socio-cultural values and ideals, which is not met in any of the other three stakeholder groups. Experimentation with technology, open software and do-it-yourself (DIY) tools, sensitivity to privacy and network neutrality, the desire to bridge the digital divide, but also commitment to the community spirit and social movement, participatory governance and decision-making, and protection of consumers' rights, count as primary motives of people that lead the CN initiatives, mixing in variable ways both across and within the different CNs. Economic incentives are also present in a few cases, albeit to a smaller extent. On the contrary, in many cases, the members of the volunteers' group end up investing a lot of personal effort, time, and money to the CN initiative, without direct financial return of any kind.

The incentives of the volunteer groups are not necessarily static throughout the lifetime of the CN initiatives. There are instances where these have evolved over time, adapting to the group membership (\eg members joining or leaving the group), new technologies that were made available over time, and the evolution of the surrounding legal/regulatory environment.

\subsubsection{Political incentives}\label{subsec:vol_political}
Political causes often serve as driving forces for the groups that lead CN initiatives. A characteristic example of principles underlying such initiatives is found in the declaration by the guifi.net foundation, the volunteers' group that has developed and still operates the guifi CN, in Catalunia, Spain ~\cite{Perez2016, barcelo2014bottom, 5514608}:
\begin{itemize}
\item Freedom to use the network, as long the other users, the contents, and the network itself are respected.
\item Freedom to learn the working details of network elements and the network as a whole. 
\item Freedom to disseminate the knowledge and the spirit of the network.
\item Freedom to offer services and contents. 
%\item By joining the network, the network is extended according to the previous principles. 
\end{itemize}


Such causes often prove to be strong enough to fuel these groups' active involvement with the CN despite the effort, time and money this requires.% and the participation fatigue.% phenomena %described in \cref{subsec:fatigue}. We list the most important of such causes in what follows.


\begin{description}
\item[Bridging the digital divide:]

CNs have thrived in rural areas where the access to the Internet, and ICT services more generally, was (and, in many cases, still is) poor or non existent. The main reason for this is the reluctance of commercial operators to invest on fixed broadband infrastructure in remote, sparsely populated areas, because they do not deem this cost-efficient. Internet connectivity alternatives based on wireless technologies (satellite Internet, cellular data), when they are available, are usually either expensive and/or of lower quality.

The right to (broadband) connectivity is a matter of equal opportunities in the contemporary digital society; and digital illiteracy puts at disadvantage populations deprived of it. The launch of CN initiatives has many times been the response to this threat. Interestingly, the volunteers' group is not always formed by local residents suffering the digital divide (as the case is with the B4RN~\cite{NETCOMMONS_D2_2} and guifi networks~\cite{NETCOMMONS_D1_2}), but also visitors or people with origins from the area under question, as the case is with the i4Free and Sarantaporo.gr networks, respectively. More analytically \cite{NETCOMMONS_D1_2}, \cite{NETCOMMONS_D2_2}, \cite{NETCOMMONS_D2_3}:

\begin{itemize} 
\item \textbf{guifi.net} started in Osona, a village in Catalunia, in 2004. A group of people decided to create a network that would serve remote rural areas. Internet connection through conventional ISPs was not available due to the high cost related to the network deployment. The locals then, decided to solve the problem themselves by creating a wireless network throughout the region. 

\item \textbf{Sarantaporo.gr}. People with origins from the area of Sarantaporo in north-western Greece, and residents of Athens and abroad, originally wanted to create a website for the village. Yet, to their surprise, they realized that there was no network connection other than telephone modems and cellular data. This led a small group of people to put efforts and build a wireless community network. With the help of the Greek Foundation for open-source Software and local academic institutions, as well as funding from EU RnD projects, the network grew over time to cover currently 14 villages in the broader area and get used by much of the local population. 

 \textbf{i4Free}\footnote{\url{https://openhardware.ellak.gr/tag/i4free-gr/}}\footnote{\url{https://www.facebook.com/i4free.gr/}}. This is a network that started from the initiative of a German engineer and professor in an island of Greece with poor Internet connectivity. Anticipating the importance of Internet resources and equipped with technical knowledge, the initiator of i4free created a small network at his own expenses so that locals could have access to ICT services.%\todo{weblink to i4free?} It does not actually have a web page of its own. We've provided links of its facebook page and the reference to it from the open hardware group. 

\item \textbf{B4RN}. The Broadband For Rural North (B4RN) initiative in Lancashire, UK, aimed at bridging the digital divide, started in December of 2011 by a local volunteer group led by a networking expert, Barry Forde. Contrary to other CNs, their CN is based exclusively on fiber and was developed as a more affordable and cost-efficient alternative to broadband access than alternative technologies such as satellite and cellular. 
\end{itemize}

%For all these cited CNs netCommons Deliverable D1.2\,\cite{NETCOMMONS_D1_2} and D2.2\,\cite{NETCOMMONS_D2_2} report details and analysis on their structure and motivations. 







\item[ Openness, net neutrality, and  privacy:] 
\label{net_privacy}


These highly controversial subjects have served as primary motivations for CN initiatives. The principle of net neutrality dictates that traffic within the network should be treated in an equal manner independently of the content or the source. The data that is communicated across the network is not subject to discrimination. However, this is not the case in the Internet where large ISPs are able to block and prioritize traffic without having the consensus to do so~\cite{dischinger_2010, miorandi_2013, dischinger_2008}, often also disregarding basic legislation on freedom of communications.  

 Moreover, volunteers are often interested in accessing ICT services without having to compromise their \textbf{privacy}. This applies for technology enthusiasts, activists and users in general that wish to protect their private content. 
 %Due to the nature of a CN, the risk of having data that is being monitored is small when compared to the corresponding risk when navigating the Internet. The Free Network foundation, the DarkNet are examples of privacy preserving initiatives~\cite{Hodson201320}
 
CNs such as the French FFDN and the German Freifunk declare privacy/anonymity and net neutrality as integral parts of their manifesto and incorporate them in their fundamental operation principles. 

\begin{itemize} 
\item The \textbf{FFDN}\footnote{\url{https://www.ffdn.org/}.} was founded in 2011 as an umbrella organization embracing 28 CNs operating across France (plus one in Brussels, Belgium), including the most popular French CN by that time, FDN. This happened after a a call by FDN's president Benjamin Bayart and other FDN active volunteers to people across France to start building their CNs. This call came as a response to several events that made an impact on the debate about digital rights (\eg WikiLeaks, Cablegate,DataGate). All CNs under the FFDN association adhere to values of collaboration, openness and support of human rights (freedom of expression, privacy) embedded by the Free Software Movement. %\todo{DataGate?}

\item \textbf{Freifunk} is an open initiative that supports free computer networks in the German region,  counting about 150 local communities with more than 35,000 access points. It started its operation in Berlin attracting many artists, activists and tech enthusiasts from all over Europe. The incentives behind its initiative are reflected in the very early statement of its basic principles of operation: (a) Public and anonymous access; (b) Lack of commercial flavor and censorship; (c) Decentralized operation and community ownership over it.

\end{itemize}

\item[Autonomy and alternative communication models:]
These are common motives for the original deployment and subsequent operation of CNs~\cite{lawrence2007wireless}, especially in urban areas, where the digital divide threat is much less pronounced. Community networks such as  Consume\footnote{\url{http://consume.net/}}\footnote{\url{http://wiki.p2pfoundation.net/Consume}} and Free2Air\footnote{\url{http://www.free2air.org/}}\footnote{\url{http://wiki.p2pfoundation.net/Free2Air}} started out representing alternative approaches to the commercial Internet provision, aiming at higher freedom and control over personal communications. In other cases, such as guifi.net, which started as an attempt to bridge the digital divide, such political purposes emerged as an equally strong motivation factor, especially when the number of network connectivity alternatives increased. In more detail:

\begin{itemize} 
\item \textbf{Consume.} This CN was one of the first ones to be conceived and deployed in Europe. Its development was led by James Stevens and Julian Priest and a number of people that were organized around them. Although the original motivation was to save Internet access fees for conducting business, the initiative evolved to an attempt to ``short-circuit" what, by that time, has become the {\it ``anti-competitive telecommunications market model''}~\cite{NETCOMMONS_D2_2}. 

\item \textbf{Free2Air.} This initiative was initiated in East London as an alternative network to the commercial Internet provision. The initiative was run by a small number of artists and a number of other individuals, a central figure being Adam Burns, an IT security expert. Himself together with a few others set up the network addressing the main technical tasks such as network routing, planning, and other tasks. Burns describes Free2Air as a largely political project, attempting to put into practice ideas about control and ownership of personal communication. He recalls that the one of the two main motivations for starting the network was exactly to try de-mediating the personal communication and getting more control over the communication needs~\cite{NETCOMMONS_D2_2}. Burns himself was involved in significant political activities participating in debates on the idea of commons and what this implies for governance, legal and policy issues, but also the alternative organization and autonomy of communication. 

\item \textbf{guifi.net.}  Guifi CN has formalized its alternative approach to network operation and management in the context of the economic theory of Commons. The guifi.net foundation promotes the view of their CN as CPR and apply principles of CPR management, as set by the Nobelist economist Elinor Ostrom~\cite{Ostrom1990}, to their CN management. 
\end{itemize}

\end{description}



\subsubsection{Socio-cultural incentives}
Socio-cultural motives are strongly relevant to the participation of volunteer groups in CN initiatives. There are instances that such motives stand behind the original conception and deployment of CNs; in other cases, these may emerge in a later stage across the people who run and manage the CN.  

Concepts of intrinsic motivation such as \textbf{creativity, innovation}, enjoyment are found in the group of volunteers in CNs. Education and knowledge acquired from the interaction with other network members and involvement with the network\,\cite{4124126}, tend to be noted and appreciated by the members of a CN. 


\begin{description}
\item[Experimentation technology and DIY culture:]
Several initiatives are driven by hackers, technology enthusiasts, and academics who enjoy experimenting with network and radio technologies. The involvement within such a community presents them with a unique opportunity to further enhance their technical knowledge and practise it over real networks.

\begin{itemize}
\item \textbf{AWMN.} The AWMN was founded in 2002 by a group of people involving primarily network technicians and enthusiasts and radio amateurs. The network was characterized by a culture of experimentation and improvisation \cite{NETCOMMONS_D2_2}.
For the people leading the activity, it was a great place to test and enhance their knowledge and create things. This involved the manufacturing of antennae, the production of feeders, and the design of mesh protocols for routing traffic over the network.

This experimentation and hacking culture is best reflected in the unparalleled offer of applications and services that were developed for AWMN, \ie to work as native services without need for public Internet connectivity, including games, libraries, network monitoring tools, DNS solutions, and experimental platforms.

\item \textbf{Ninux.} Experimentation and hacking were the primary motivation behind setting up the Ninux CN in Italy early 2000s. This is directly reflected in its name, as ``Ninux" stands for "No Internet, Network Under eXperiment". As with AWMN, Internet access is not officially offered by Ninux, which operates as an experimental platform for decentralized protocols, policies and technologies.

\item \textbf{Funkfeuer.} Funkfeuer is a free experimental wireless network across Austria. It was built and currently maintained by a group of computer enthusiasts with different motivation and interests. Funkfeuer is committed to the idea of DIY. 
\end{itemize}

\item[Community spirit and altruism:] 

Altruism, often coupled with belief in community ideals emerge as important motivations for the active involvement of volunteers' groups in CNs.

\begin{itemize}
\item \textbf{B4RN.} The community ideals are highly prioritized in B4RN. The volunteer group has been set up to operate as a community benefit society which “can never be bought by a commercial operator and its profits can only be distributed to the community.” This was a decision early made by the few people who initiated the CN. 

\item \textbf{Sarantaporo.gr.} The Sarantaporo.gr involves people who are activists in the area of commons and supporters of community ideals. They place a lot of emphasis on cultivating these ideals in the residents of the area with parallel activities and social events. Even the small yearly subscriptions that aim at the maintenance of the network infrastructure are determined at village/community rather than individual level.

\item \textbf{i4Free.} The leading figure behind the i4Free CN in Greece, is also a warm fan of community life and ideals. He has spent enormous amounts of time in training and educational events trying to build a community around the CN, even without much success as he admits \cite{NETCOMMONS_D2_2}.

\end{itemize}

Altruism and the spirit of community are also evidenced in other CNs, where the primary motivation of volunteers is the experimentation and hacking culture or other political reasons.% (see %\cref{subsec:vol_political}). 
Therefore, in AWMN and Ninux, guides and instructions have been developed with the certain purpose of providing information and recommendations to interested potential participants in order to buy and set up their own node. 


\end{description}

\subsubsection{Economic incentives} \label{subsec:vol_economic}



Economic incentives are rarely relevant to the volunteers' group. These groups are mostly organized as nonprofit organizations and, in several cases, their members end up funding the initiative one way or another. Yet, there are some instances that such incentives are present, or were present at some stage of the CN development. In all cases, the underlying idea, when present, is how to save money with CNs compared to commercial alternatives rather than how to make money out of the CN initiative.

\begin{itemize}
\item \textbf{Consume.} One such case is the Consume network, one of the very first CN initiatives that set a recipe for other CNs across Europe. James Stevens ran a technology incubation business offering web, live streaming and video distribution services through a leased optic fiber connection. He came up with the idea to connect buildings through wireless mesh links as a way to bypass the expensive licence costs and regulatory constraints related to expanding the fiber communication across the buildings.

Yet, the initiative soon acquired more political purposes, as a movement against anti-competitive practices that protected certain financial monopolistic interests in UK. And the two people that led the development of the network, Stevens and Julian Priest, ended up undertaking almost the full financial cost related to the network deployment.

\item \textbf{BARN.} In the rural areas covered by B4RN, there is no fixed commercial broadband infrastructure available since commercial operators do not consider it worth in financial terms. Yet, there are other options such as satellite or cellular 
that are typically more expensive and of lower quality. B4RN offers better connections at more affordable prices than the competing solutions.

\item \textbf{Ninux.} Indirect economic benefits can come through the enhancement of an individuals human capital. From their involvement with the network, individuals in Ninux have acquired knowledge needed to find jobs in the ICT sector.

\end{itemize}








\subsection{Users} 



Users are people that join the network for different kind of reasons. Their reasons for participating may refer to network access, acquiring connectivity and utilizing the resources of the network for data exchange, communication or gaming. A user can either pay a fee for connecting to the network or not. Examples of both cases are found in practice i.e. in different CNs or even within the same CN. It is also possible for users to join the network for non-technical reasons. Some may be interested in exercising activism while others wish to ensure data privacy. Receiving qualitative services provided by the professionals is another typical example. In cases where CN users are interested only in \textit{network access} and \textit{professional service consumption} and offer some kind of reimbursement in exchange, users are considered \textit{customers}. Practically, their participation is followed by a connectivity fee paid directly to the CN or consumption fees paid to the professionals for consuming their services and indirectly to the network.   

User participation levels exhibit high variance. They may be highly active and participate in the events organized by volunteers or other types of
collective activities, provide technical experience, develop apps, and devote personal time and efforts
to the network, get involved in the service offering of professionals and contribute to the economic activity of the CN; they may set up a node without contributing personally to the activities
of the community; or they may use the CN to get Internet access or access to local services without
contributing in any way (economic, hardware or personal efforts). The latest type of users are termed \textit{free riders}. However, their participation may benefit the network in terms of the network effect i.e. the larger the
network the easier to enter, so even passive users such as free riders can potentially enable others to join.
 

Likewise variable is their motivation for joining the CN. Decisive for many of them is the expectation of cheap, or even free, Internet access. For others, the CN is viewed as a perfect opportunity to acquire new knowledge and experiment with high tech stuff. Socializing and becoming part of a bigger community is also reported as important motivation for participation in the CN. 
Finally, political causes are also evidenced as motives for user participation, albeit to a smaller extent than in volunteer groups.

\subsubsection{Political incentives}
Although users of the network are not involved in its initial deployment and operation, they may too experience political motives for participating in the network.

Many CNs as seen in section \ref{subsec:vol_political}, have been created under aspirations of privacy and net neutrality, autonomy and self-organization, providing an alternative to existing communication models and bridging the digital divide in rural, poorly served by ICT operators, areas. 
%Sharing 
The ideals underlying the initial development of these CNs are often passed on some of their members --the larger the CN the harder to find political causes uniting the whole community behind them.

\begin{description}
\item[Openness, net neutrality and privacy:]\label{privacy_users} Users often participate in CN initiatives in an attempt to get away with privacy concerns and tracking/monitoring software used in the public Internet. 
%Even if they don't necessarily participate in the management of the network they use the network with the objective of ensuring privacy in communications and data exchange without being subject to surveillance or discrimination. 
The aspects of privacy and neutrality have a strong role in networks that utilize the Picopeering agreement\footnote{\url{http://www.picopeer.net/PPA-en.shtml}} and are part of the movement for open wireless radio networks\footnote{\url{https://openwireless.org/}}. The Picopeering agreement is a baseline template that formalizes the interaction between two peers of the network. Its basic properties include:
\begin{itemize}
\item Node owners agree on free exchange of data into, out of or across a network without any interference.
\item Node owners agree on providence of open communication by publishing relevant peering information subject to free license and information of contact.
\item There are no guarantees of service level.
\item Node owners can formulate use policies as long as they do not interfere with the basic parts of the picopeering agreement. 
\item Local amendments can take place by the will of node owners.
\end{itemize}

\item[Autonomy and self-organization:] 
The participation in CN groups cultivates feelings of autonomy and self-organization. Self organization is also depicted in the way that new users connect to the network, where they have to rely on their own resources and on the voluntary assistance of experienced network members. 

Being part of an independent network satisfies personal ideology aspirations for self-organized network and autonomous use. The ability to participate in collective decision making and contribute to the a "common" network infrastructure following an alternate model of ICT access is itself an experience for users interested in participating in a community of "commons". In the study found in~\cite{lawrence2007wireless}, 94.5\% responded that they experienced autonomy in their groups and expressed freely their own opinions. 

%Residents of the remote rural areas that can use it as an independent way to access to ICT services. Also, in order to acquire connection to the network or face technical difficulties, 

\end{description}

\subsubsection{Socio-cultural incentives}
A CN is a characteristic example of participatory involvement, where users dedicate their efforts and time to the network~\cite{Vega2014}. A number of services and applications combined with other activities that one way or another revolve around the CN, offer users the opportunity to communicate, educate and entertain themselves, thus further motivating their participation in the network ~\cite{szabo2007wireless}~\cite{pedraza2013community}. 


\begin{description}
\item[Experimentation and new ICT knowledge acquisition:] Technology enthusiasts participate in the network for experimenting with the technology and new gadgets. 
%This applies technology enthusiasts that attracted by ICT services and wish to experiment with technology, 
They find in a CN an as realistic as possible testbed for trying software they develop and hacked code, make network speed measurements, play with network mapping and management tools.

Other users view CNs as a ``place", where they can acquire new skills about computer and network use. They are willing to invest personal effort on this but, at the same time, they expect to get triggers and help and guidance from the experts that know more about this. %network members  that they will have to attend online or physical seminars, learn about the use of wireless technologies, software and hardware, routing, have access to digital libraries etc. 
AWMN, Ninux, and Freifunk are CNs built by people with solid technical background and technology lovers. It is no surprise that many of the users these CNs attract tend to share similar interests.

 
In CNs that were initiated by volunteers with technical background, the amount and type of services, applications and self-produced software increased greatly within the community. 
In such CNs, users with these kind of motives appreciate getting access to:
\begin{itemize}
  \item communication services with VOIP and forums, mails, instant messaging, 
 \item data exchange services with servers, community clouds, file sharing systems, 
  \item entertainment services with games, applications, video and audio broadcasting,
  \item information and educating services with online seminars, e-learning platforms, wikis, monitoring tools, search engines.
%  \item third party services offered by professionals, 
%  \item internet service which offers itself access to a wide variety of services. 
\end{itemize}
 
In a study found in~\cite{lawrence2007wireless}, 78\% of the people that filled in questionnaires reported that the CN satisfied their personal needs, and 87\% were identified as technology enthusiasts. 

\item[Social interaction:]
The smooth operation and development of a CN demands  cooperation links at the network infrastructure level but also at the social level. 
Works ~\cite{4468734} and ~\cite{4444315} state that the social layer in P2P+ systems is often neglected and left out of the design of incentive mechanisms. 
As social incentives count socially-aware mechanisms that may relate to concepts such as visibility, acknowledgment, social approval, individual privileges and status. This social activity is applied within the networks' technical limits~\cite{Mcdonald02socialissues}. 
 
\textit{Social motives} are common in the participation of users and affect network growth and operation~\cite{6979946, 4124126}. 
In CNs, participants are able to share their ideas and interests, participate in groups, interact and communicate with other network members just like they would in any other online or physical community. 
Communication within or outside the network is an easily observable motive and one of the most popular reasons why users take part in online communities. Social networking and communication tools raise great interest and remain active even when other tools and services have a drop in their utilization. 
Finally, the ability to compete with other people and satisfy one's self esteem through the involvement in the community, or receive a certain type of credit by others in the community, are motives not as easy to distinguish but still present in reported studies. 
 
\begin{itemize}
 \item  In the study in~\cite{lawrence2007wireless} results showed that 91.2\% enjoyed interacting with the community, 88\% felt that their efforts would be returned by other community members and 80.5\% expressed that the community allowed them to work with people that they could trust and share similar interests. 
 \item A socio-technical study in the rural area of northern Thailand, showed that CN users with access to the Internet showed great interest in messaging, email, online social networks, and online gaming services~\cite{Lertsinsrubtavee:2015:UIU:2837030.2837033}. The social activity among the users exhibited a high degree of locality, which means that people used Internet to interact with people within the same CN. 
 
 \item Similar results were found in a study of Internet service in a rural village in Zambia~\cite{Johnson:2010:IUP:1836001.1836008}. The implication is that local relationships can be of great importance in a CN~\cite{kornhybrid} and that even though Internet service is dominant in certain community networks~\cite{6673334}, if similar services could be applied at a local scale, they would have the potential to make an impact on CN users. 
\end{itemize}


\end{description}

\subsubsection{Economic incentives}
Motives of economic nature are evidenced and have been reported in literature among CN users. Namely, users expect benefits of economic nature from their participation in the network, which may be direct or indirect. 
\begin{description}
\item[Direct economic benefits:] One of the main reasons why users join CNs  is that they can get Internet access at lower cost than alternative commercial solutions, offered by telecom operators. 

\begin{itemize}
\item \textbf{Sarantaporo.gr} offers Internet connectivity at a small subscription fee that is charged on per village basis. The resulting cost per network user goes down with the number of people sharing the Internet access and is several times smaller than what the same users would need to pay if they individually subscribed to available commercial solutions. In fact, the anticipation of the CN as "Internet for free" has put a lot of obstacles towards a more participatory stance in sharing the CN operational expenses. 
%for each AP located in the various villages entails a connectivity fee per year per access point (multiple users) which is about half the amount of money required for an annual single user connection in a telecom operator. 
%\item \textbf{FFDN} members, who are actually members of the official organizations forming the alliance, pay basic membership fees separately for consumption of specific services. 

\item \textbf{AWMN} members of the Association pay a typical small subscription fee in exchange for rights and involvement in decision-making processes. Non-members of the Association are not required to pay any kind of fee except for the expenses of their own equipment.

\item One of the strong points in the evolution of \textbf{B4RN} has been its capability to offer fiber connectivity and Internet speed at much more favorable prices than alternative commercial solutions did. Part of these savings relates to partly crowdsourcing the cost and effort for digging, which is a strong indication of how these initiatives can mobilize local skills and resources.

\end{itemize}

\item[Indirect economic benefits:]

Users do not always identify economic benefits (only) with the capability to save money for Internet access. 

\begin{itemize}
\item In \textbf{Sarantaporo.gr} young people (in the age of 18-35) view the CN as a path to information about job and further education opportunities; farmers search better markets for their products and cheaper suppliers for raw materials; and locals running coffee shops or taverns join the network in the anticipation that visitors appreciate the Internet connectivity feature when choosing where to go. 

\item In \textbf{AWMN} people out of those who contributed to its development also developed some business activity around the CN. They had Wi-Fi expertise and broader technical knowledge and opened shops to provide infrastructure for the network \cite{NETCOMMONS_D2_2}.
\end{itemize}



\end{description}
\subsection{Professionals}

The professional is the stakeholder type that is most rarely met in CN initiatives.
In fact, and to the best of our knowledge, guifi.net has been the first and single CN instance with clear
and well articulated provisions for the involvement of professionals in the CN ~\cite{Baig:2016:MCN:2940157.2940163}.
At first glance, these entities do over the CN what they do over any other network. However, the legal provisions and conditions of running business over the CN
are different. In the case of the guifi CN, the guifi.net foundation prepares licences that serve the
commons purposes and ensure that any professional entity providing service over the network will also contribute to the network expansion and maintenance ~\cite{Baig2015150}.


  The CN is a great opportunity for users to receive services. Services may include Internet access, cloud storage, video streaming and video on-demand. They are offered by professionals who come into touch with the users via the infrastructure of the network. Professionals are usually companies, ISPs, small businesses or individuals, i.e., entities that use the network to provide commercial services, promote their expertise in a specific field and get compensated for it. In contrast to the traditional telecommunication companies where users are seen solely as consumers, users in CN can themselves become professionals and take part in the service provision. 

Their main focus of the professionals is \textit{demand, service supply and stability of operation}. \textit{Demand} stands for finding customers in need of their offers within the network. For example the expansion of the network is usually beneficial for the professionals, because it increases their potential customers. However, it may also increase the competition. The \textit{service supply} is the principal role of the professionals for network users. They are also interested in the quality of their service they provide to the end customers, as it is their main distinguishable feature within the network's market. \textit{Stability of operation} is inherently interconnected to the networks operation. For professionals to be able to provide a qualitative and stable service the network has to provide uninterrupted network connection for both the professionals and the users. But they are not independent from the CN. Professionals contribute to the technical infrastructure directly by contributing actual hardware or indirectly by providing economic contributions. In this way, they have a slice of responsibility for the network operation as they are themselves part of it. 








The incentives for the participation of professionals in the network are primarily, if not exclusively, economic.
\subsubsection{Economic incentives} 

\begin{itemize}
\item The most advanced network so far, is the \textbf{guifi.net} which incorporates a number of organizational rules to promote economic interaction within the network and motivate professionals to participate and offer their services using the CN technical infrastructure. Professionals are able to participate in the network, provide their services over it and get compensated for them. 

\item \textbf{B4RN}, a fiber community network located in Lancashire in England, employs a community funding model composed of shares for each investment, support for loans from the community and subscription fees for the participants. Community members can acquire B4RN shares. The network's expenses are covered by its own shareholders. B4RN utilizes a subscription model for both households and non domestic users. The subscription model is composed of a connectivity fee and different service fees for different types of users. 

\end{itemize}


\subsection{Public administrations} 

Public administrations may interact with a CN in different ways: 
\begin{itemize}
\item by contributing to the deployment and growth of the CN through either funding the initiative or sponsoring network equipment. 

\item by positioning as a user of the CN services. In case of municipal authorities, they might let a CN manage and maintain equipment they own in return for network connectivity. 

\item as a regulating body facilitating or placing obstacles to its expansion and growth or by permitting the use of public space and resources by a CN (\eg as antenna or CN node installation sites)
\end{itemize}


It is possible to distinguish other types of groups that may get involved in the network such as Universities and other organizations. Depending on their level of participation they can sign collaboration agreements with the legal entity of the CN and contribute economic or infrastructure resources with or without compensation. 

\subsubsection{Political incentives}
Public bodies may serve different political causes by participating in a CN and/or funding its activities.

First of all, it is possible to implement EU promoted policies against the digital divide and in favor of equal opportunities in the digital economy and society. CNs have shown over time their potential to mobilize local communities and altruistic forces in the society. They have managed to offer network connectivity in areas that are not attractive for commercial operators and might otherwise need generous public subsidies to cover. Second, the CNs often strengthen the community links and raise awareness for issues concerning the local societies. Ideally, CNs sort of train users to become more engaged with the commons. Third, on a more selfish and short-sighted note, local administrations (such as municipalities) can advertise the provision of network services as a political achievement that increases their chances of re-election. 
%\todo{can mention EC prizes given to CNs here} \todo{Not sure how this fits the political incentives.}



\begin{itemize}
\item \textbf {Sarantaporo.gr} The Greek Foundation for open-source software, an initiative with the participation and support of the whole Greek academia, has sponsored the network equipment for the initial deployment of the CN in 2013. The University of Applied Sciences of Thessaly has provided them with connectivity to the Internet through its access to the Greek Research and Education Network (GRNET). Additional funds through the participation in the EU FP7 CONFINE project allowed the network expansion to 14 villages in the area.

\item \textbf{guifi.net} The local authorities of many villages in Catalunia have allowed the foundation to dig public space and lay down fiber for expanding the network coverage to these areas.

\end{itemize}

\subsubsection{Economic incentives} 
Public administrations can participate in the network because this may prove profitable, just like professional entities do. 

\begin{itemize}
\item \textbf{guifi.net} In the case of guifi.net public administrations can fund the network expansion through purchase of equipment in return for added value services over the network. In other words, they can invest in the network and get compensated for their investment.
\end{itemize}

\begin{center} 

\begin{table*}[t]
\centering
\resizebox{12cm}{!} {
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{CN} & \textbf{Location} & \textbf{Creation} & \textbf{Initiators}  \\
\hline
   AWMN &  Athens, Greece  &     &   \\
  \hline
  B4RN  &  Lancashire, UK &  &  \\
  \hline
  Consume & London, UK &    & \\
  \hline 
  FFDN &  France, Belgium &  & \\ 
  \hline 
  Free2Air &  London, UK &   &\\
  \hline
  Freifunk &  Berlin, Germany &   & \\
    \hline
 Funkfeuer &  &    &  \\ 
  \hline 
  guifi.net & Catalonia, Spain &    & \\
  \hline 
  i4Free &  Fokida, Greece &    & \\
  \hline 
  Ninux &  Italy    &   &\\
  \hline 
  Sarantaporo.gr & Elassona, Greece  &  &\\
  \hline 
\end{tabular}
}
\caption{Community networks studied here.}
\end{table*}

\label{tab:mechanism_stakeholder}
\end{center}

